Resource-Efficient Semantic Communication for Heterogeneous Agentic Teams

Teams of autonomous agents, including large language model (LLM) agents, must coordinate over scarce and unreliable wireless links. We propose goal-oriented semantic communication (GOSC), a closed-loop co-design that jointly decides what each agent sends, when it sends it, and how reliably it is transmitted, based on each message's value to the team task. An edge broadcast of the team's common knowledge closes the loop by updating these values. We prove that a message is sent only if its value exceeds the cost of delivering it and that more valuable messages receive more robust transmission rates, and we show that the scheduler solves each scheduling step exactly whenever the radio budget is not saturated, which held in 95% of scheduling decisions. In search-and-rescue missions validated on unseen scenarios, GOSC meets the same mission targets as carefully tuned periodic semantic schemes with 1.2--8.5 times fewer uplink channel uses. In most settings, this advantage persists with realistic packet overheads, reaching 16.6 times fewer uplink channel uses and 13.8 times lower cost when downlink costs are included; in the rescue task, it also persists when all agents share one uplink. Rough value estimates suffice, whereas values that ignore message content can fail. With three different LLMs, GOSC uses 3.2--3.5 times fewer channel uses, while completion-time gains depend on the model.

==> figures/table_ablation.tex <==
100 & \textbf{GOSC (ToM VoI + filter)} & 72.9 $\pm$ 6.0 & 12.1 & -- \\
 & ToM VoI, no filter & 70.6 $\pm$ 4.8 & 12.3 & -2.3 [-7.8, +3.1] \\
 & Throughput value + filter & 68.9 $\pm$ 5.8 & 26.2 & -4.0 [-11.5, +3.8] \\
 & Throughput value, no filter & 70.1 $\pm$ 4.4 & 33.7 & -2.8 [-9.9, +4.1] \\
 & ToM VoI + filter, conventional link adaptation & 88.7 $\pm$ 8.2 & 8.0 & +15.8 [+7.7, +24.2] \\
\midrule
50 & \textbf{GOSC (ToM VoI + filter)} & 78.4 $\pm$ 7.5 & 7.2 & -- \\
 & ToM VoI, no filter & 86.4 $\pm$ 9.8 & 7.4 & +8.0 [-1.1, +17.7] \\
 & Throughput value + filter & 74.6 $\pm$ 5.9 & 16.8 & -3.8 [-12.3, +4.8] \\
 & Throughput value, no filter & 78.6 $\pm$ 6.0 & 19.8 & +0.1 [-8.8, +9.2] \\
 & ToM VoI + filter, conventional link adaptation & 88.4 $\pm$ 9.0 & 5.0 & +10.0 [-0.8, +20.2] \\


==> figures/table_cost_r2.tex <==
\multicolumn{7}{@{}l}{\emph{Overhead $H=0$ bits}}\\
\quad Report only & 187.9 & 0.7 & 0.0 & 0.1 & 0.0 & 0.8 \\
\quad Raw sensor data & 152.7 & 90.7 & 0.0 & 5.6 & 0.5 & 96.7 \\
\quad Natural language & 142.2 & 85.3 & 0.0 & 7.5 & 0.4 & 93.3 \\
\quad Semantic periodic & 78.3 & 41.1 & 0.0 & 6.0 & 0.2 & 47.4 \\
\quad Best periodic (rate-aware + filter) & 76.2 & 14.0 & 0.0 & 3.7 & 0.1 & 17.8 \\
\quad \textbf{GOSC} & 70.9 & 11.8 & 0.0 & 3.3 & 0.1 & 15.2 \\
\midrule
\multicolumn{7}{@{}l}{\emph{Overhead $H=32$ bits}}\\
\quad Report only & 187.0 & 1.2 & 0.4 & 0.2 & 0.0 & 1.5 \\
\quad Raw sensor data & 165.4 & 98.5 & 31.8 & 4.9 & 0.5 & 103.8 \\
\quad Natural language & 186.5 & 111.9 & 35.8 & 6.6 & 0.6 & 119.1 \\
\quad Semantic periodic & 89.5 & 49.4 & 17.2 & 4.6 & 0.3 & 54.2 \\
\quad Best periodic (rate-aware + filter) & 72.2 & 23.9 & 9.6 & 5.4 & 0.2 & 29.5 \\
\quad \textbf{GOSC}$^\dagger$ & 79.8 & 14.8 & 6.4 & 3.9 & 0.1 & 18.8 \\


==> figures/table_default.tex <==
Report only & 188.6 $\pm$ 16.9 & +115.7 [+98.5, +133.7] & 0.19 & 0.66 & 0.17 & 0.12 \\
Raw sensor data & 133.7 $\pm$ 11.6 & +60.9 [+48.1, +74.2] & 29.63 & 79.33 & 0.22 & 0.07 \\
Natural language (LLM-style) & 150.6 $\pm$ 9.9 & +77.7 [+67.7, +88.3] & 41.02 & 90.35 & 32.82 & 0.09 \\
Semantic, periodic & 78.7 $\pm$ 6.4 & +5.8 [-2.4, +13.8] & 15.71 & 41.30 & 0.21 & 0.02 \\
\textbf{GOSC (proposed)} & 72.9 $\pm$ 6.0 & -- & 12.05 & 12.06 & 0.21 & 0.06 \\
\midrule
Ideal-comm. reference (genie) & 61.0 $\pm$ 3.5 & -11.9 [-19.0, -5.1] & 17.68 & 0.00 & 0.00 & 0.02 \\


==> figures/table_efficiency.tex <==
Search & $T\le1.15\,T_{\mathrm{g}}$ & 17.3 & 15.0 & 1.2 [0.8, 1.9] (98\%) & 1.0 [0.6, 1.8] (86\%) \\
Search & $T\le1.25\,T_{\mathrm{g}}$ & 14.0 & 8.8 & 1.6 [1.0, 2.5] (100\%) & 1.4 [0.9, 2.2] (100\%) \\
Search, $W{=}50$ & $T\le1.15\,T_{\mathrm{g}}$ & -- & -- & -- & -- \\
Search, $W{=}50$ & $T\le1.25\,T_{\mathrm{g}}$ & 12.5 & 12.7 & 1.0 [0.8, 2.4] (84\%) & 0.7 [0.7, 1.7] (76\%) \\
Search, $K{=}10$ & $T\le1.15\,T_{\mathrm{g}}$ & 22.8 & 3.9 & 5.8 [1.4, 10.2] (100\%) & 2.3 [0.8, 8.8] (98\%) \\
Search, $K{=}10$ & $T\le1.25\,T_{\mathrm{g}}$ & 14.2 & 2.0 & 6.9 [3.8, 10.3] (100\%) & 5.9 [2.9, 12.2] (100\%) \\
Search, clustered & $T\le1.15\,T_{\mathrm{g}}$ & 8.8 & 7.4 & 1.2 [0.8, 1.7] (100\%) & 1.5 [0.8, 2.4] (100\%) \\
Search, clustered & $T\le1.25\,T_{\mathrm{g}}$ & 7.6 & 5.7 & 1.3 [0.9, 1.9] (100\%) & 1.9 [1.2, 3.3] (100\%) \\
\midrule
Rescue & $S\ge0.90\,S_{\mathrm{g}}$ & 6.8 & 4.4 & $\ge$1.6 [1.3, 2.5] (100\%) & $\ge$4.6 [3.9, 7.5] (100\%) \\
Rescue & $S\ge1.00\,S_{\mathrm{g}}$ & 16.0 & 20.1 & 0.8 [0.7, 2.4] (98\%) & 1.1 [0.7, 2.1] (96\%) \\
Rescue, $W{=}50$ & $S\ge0.90\,S_{\mathrm{g}}$ & 7.2 & 3.3 & $\ge$2.2 [1.7, 3.4] (100\%) & $\ge$6.6 [5.2, 10.2] (100\%) \\
Rescue, $W{=}50$ & $S\ge1.00\,S_{\mathrm{g}}$ & -- & -- & -- & -- \\
Rescue, $-5$\,dB & $S\ge0.90\,S_{\mathrm{g}}$ & 43.8 & 5.2 & $\ge$8.4 [5.4, 9.2] (100\%) & $\ge$15.3 [9.8, 16.8] (100\%) \\
Rescue, $-5$\,dB & $S\ge1.00\,S_{\mathrm{g}}$ & -- & -- & -- & -- \\


==> figures/table_fidelity.tex <==
Theory-of-mind VoI & +0.00 [-0.14, +0.11] & +0.05 [-0.05, +0.15] & +0.04 [-0.06, +0.14] \\
Belief divergence & +0.01 [-0.15, +0.13] & +0.08 [-0.02, +0.17] & +0.07 [-0.02, +0.15] \\
Throughput (bits) & +0.10 [-0.11, +0.13] & +0.08 [-0.03, +0.18] & +0.06 [-0.04, +0.15] \\
Age of information & +0.11 [-0.12, +0.14] & +0.08 [-0.03, +0.16] & +0.04 [-0.07, +0.12] \\


==> figures/table_frontier.tex <==
100 & 5k & 86.4 & +13.4 [+5.4, +23.4] & -0.3 [-8.0, +8.1] & -- \\
100 & 10k & 74.8 & +12.0 [+4.2, +21.3] & +1.3 [-5.6, +7.7] & +2.6 [-4.5, +19.6] \\
100 & 20k & 66.4 & +6.9 [+1.9, +12.0] & +3.4 [-2.7, +8.1] & +1.7 [-3.8, +6.0] \\
\midrule
50 & 5k & 87.0 & +16.5 [+6.3, +27.5] & -1.6 [-9.9, +8.4] & -- \\
50 & 10k & 78.4 & +13.4 [-0.5, +26.2] & +2.0 [-4.8, +11.4] & +2.9 [-6.2, +14.8] \\


==> figures/table_frozen.tex <==
Search & $\eta=10^{-5}$ & rate-aware + filter, $k{=}4$ \\
Search, $K{=}10$ & $\eta=3\cdot10^{-4}$ & suppressing, $k{=}4$, $\theta{=}0.05$ \\
Search, clustered & $\eta=3\cdot10^{-5}$ & suppressing, $k{=}4$, $\theta{=}0.2$ \\
Rescue & $\eta=10^{-4}$ & suppressing, $k{=}2$, $\theta{=}1.0$ \\
Rescue, $W{=}50$ & $\eta=10^{-4}$ & suppressing, $k{=}2$, $\theta{=}1.0$ \\
Rescue, $-5$\,dB & $\eta=10^{-4}$ & suppressing, $k{=}2$, $\theta{=}1.0$ \\


==> figures/table_llm.tex <==
Planner only (50) & Semantic, periodic & 69.2 $\pm$ 7.3 & 35.8 \\
 & \textbf{GOSC} & 72.9 $\pm$ 8.6 & 12.0 \\
 & Genie & 63.4 $\pm$ 5.2 & -- \\
\midrule
Mixed, Qwen2.5-3B (50) & Semantic, periodic & 95.2 $\pm$ 10.7 & 49.7 \\
 & \textbf{GOSC} & 81.4 $\pm$ 8.0 & 14.2 \\
 & Genie & 76.0 $\pm$ 7.0 & -- \\
\midrule
Mixed, Llama-3.2-3B (30) & Semantic, periodic & 98.9 $\pm$ 18.0 & 52.8 \\
 & \textbf{GOSC} & 81.6 $\pm$ 12.3 & 14.7 \\
 & Genie & 76.7 $\pm$ 9.7 & -- \\


==> figures/table_llm_r2.tex <==
Planner only (50) & Semantic, periodic & 69.2 $\pm$ 7.3 & 35.8 & \multirow{2}{*}{-3.7 [-14.1, +7.0]} & \multirow{2}{*}{2.98}\\
 & \textbf{GOSC} & 72.9 $\pm$ 8.6 & 12.0 & & \\
 & Genie & 63.4 $\pm$ 5.2 & -- & & \\
\midrule
Mixed, Qwen2.5-3B (50) & Semantic, periodic & 95.2 $\pm$ 10.7 & 49.7 & \multirow{2}{*}{+13.8 [+0.8, +26.9]} & \multirow{2}{*}{3.51}\\
 & \textbf{GOSC} & 81.4 $\pm$ 8.0 & 14.2 & & \\
 & Genie & 76.0 $\pm$ 7.0 & -- & & \\
\midrule
Mixed, Llama-3.2-3B (50) & Semantic, periodic & 93.0 $\pm$ 12.6 & 49.7 & \multirow{2}{*}{+14.2 [+0.8, +28.2]} & \multirow{2}{*}{3.51}\\
 & \textbf{GOSC} & 78.8 $\pm$ 9.2 & 14.2 & & \\
 & Genie & 73.6 $\pm$ 6.9 & -- & & \\
\midrule
Mixed, Qwen2.5-7B (30) & Semantic, periodic & 99.2 $\pm$ 13.0 & 51.2 & \multirow{2}{*}{+5.2 [-11.2, +21.5]} & \multirow{2}{*}{3.24}\\
 & \textbf{GOSC} & 94.0 $\pm$ 10.8 & 15.8 & & \\


==> figures/table_noise_r2.tex <==
Exact ToM value & 1.00 & 1.19\,{\scriptsize[1.11, 1.27]} & 5.91\,{\scriptsize[5.57, 6.29]} & 1.28\,{\scriptsize[1.14, 1.43]} & 5.89\,{\scriptsize[5.44, 6.38]} & 4.43\,{\scriptsize[4.12, 4.78]} & 13.02\,{\scriptsize[11.86, 14.22]}$^\dagger$ \\
\midrule
Log-normal error, $\sigma{=}0.5$ & 0.99 & 1.75\,{\scriptsize[1.62, 1.89]} & 4.77\,{\scriptsize[4.50, 5.08]} & 1.22\,{\scriptsize[1.08, 1.37]} & 5.17\,{\scriptsize[4.73, 5.64]} & 6.84\,{\scriptsize[6.31, 7.40]} & 12.73\,{\scriptsize[11.66, 13.84]} \\
Log-normal error, $\sigma{=}1$ & 0.95 & 0.61\,{\scriptsize[0.57, 0.65]} & 3.29\,{\scriptsize[3.06, 3.53]} & 1.06\,{\scriptsize[0.94, 1.18]} & 3.67\,{\scriptsize[3.38, 3.96]} & 5.26\,{\scriptsize[4.89, 5.63]} & 12.23\,{\scriptsize[11.16, 13.34]} \\
Order of magnitude only & 0.95 & 1.15\,{\scriptsize[1.08, 1.22]} & 9.79\,{\scriptsize[9.19, 10.44]}$^\dagger$ & 1.04\,{\scriptsize[0.94, 1.15]} & 5.18\,{\scriptsize[4.69, 5.71]} & 4.40\,{\scriptsize[4.09, 4.73]} & 12.53\,{\scriptsize[11.42, 13.67]} \\
Log-normal error, $\sigma{=}2$ & 0.89 & 1.27\,{\scriptsize[1.19, 1.35]} & 3.32\,{\scriptsize[3.08, 3.58]} & 1.26\,{\scriptsize[1.12, 1.41]} & 1.84\,{\scriptsize[1.70, 1.97]} & 3.02\,{\scriptsize[2.85, 3.22]} & 9.59\,{\scriptsize[8.86, 10.32]} \\
Content-independent (permuted) & 0.14 & 0.57\,{\scriptsize[0.54, 0.60]} & 1.33\,{\scriptsize[1.23, 1.43]} & 1.27\,{\scriptsize[1.13, 1.44]}$^\dagger$ & 2.11\,{\scriptsize[1.95, 2.27]} & 3.22\,{\scriptsize[3.02, 3.43]} & 7.11\,{\scriptsize[6.60, 7.63]} \\
Permuted, no relevance filter & 0.14 & 0.46\,{\scriptsize[0.43, 0.49]} & 0.81\,{\scriptsize[0.75, 0.88]} & 1.32\,{\scriptsize[1.18, 1.48]} & 1.98\,{\scriptsize[1.84, 2.12]} & 3.24\,{\scriptsize[3.06, 3.43]} & 7.22\,{\scriptsize[6.69, 7.77]} \\


==> figures/table_overhead_r2.tex <==
\multicolumn{5}{@{}l}{\emph{Uplink channel uses, periodic / GOSC}}\\
\quad Search & 1.19\,{\scriptsize[1.11, 1.27]}$^\ddagger$ & 0.84\,{\scriptsize[0.77, 0.91]} & 1.62\,{\scriptsize[1.51, 1.73]}$^\dagger$ & only GOSC \\
\quad Search, $K{=}10$ & 5.91\,{\scriptsize[5.57, 6.29]}$^\ddagger$ & 1.86\,{\scriptsize[1.74, 1.98]} & 3.96\,{\scriptsize[3.68, 4.26]} & 2.49\,{\scriptsize[2.30, 2.69]} \\
\quad Search, clustered & 1.28\,{\scriptsize[1.14, 1.43]} & 1.46\,{\scriptsize[1.31, 1.62]}$^\dagger$ & 1.12\,{\scriptsize[1.01, 1.24]}$^\ddagger$ & 1.22\,{\scriptsize[1.10, 1.35]} \\
\quad Rescue & 1.78\,{\scriptsize[1.63, 1.93]} & 2.49\,{\scriptsize[2.18, 2.78]} & 3.01\,{\scriptsize[2.77, 3.28]} & 4.14\,{\scriptsize[3.92, 4.38]} \\
\quad Rescue, $W{=}50$ & 2.60\,{\scriptsize[2.42, 2.77]} & 3.86\,{\scriptsize[3.59, 4.13]} & 4.72\,{\scriptsize[4.42, 5.02]} & 6.04\,{\scriptsize[5.59, 6.50]} \\
\quad Rescue, $-5$\,dB & 8.52\,{\scriptsize[7.89, 9.19]} & 10.73\,{\scriptsize[9.95, 11.59]}$^\ddagger$ & 8.28\,{\scriptsize[7.60, 9.00]} & 16.61\,{\scriptsize[15.03, 18.44]} \\
\midrule
\multicolumn{5}{@{}l}{\emph{Uplink + downlink channel uses, periodic / GOSC}}\\
\quad Search & 1.17\,{\scriptsize[1.09, 1.25]}$^\ddagger$ & 0.88\,{\scriptsize[0.81, 0.95]} & 1.57\,{\scriptsize[1.47, 1.68]}$^\dagger$ & only GOSC \\
\quad Search, $K{=}10$ & 4.61\,{\scriptsize[4.36, 4.87]}$^\ddagger$ & 1.76\,{\scriptsize[1.66, 1.87]} & 3.43\,{\scriptsize[3.20, 3.67]} & 2.28\,{\scriptsize[2.11, 2.46]} \\
\quad Search, clustered & 1.22\,{\scriptsize[1.10, 1.35]} & 1.36\,{\scriptsize[1.22, 1.50]}$^\dagger$ & 1.08\,{\scriptsize[0.98, 1.20]}$^\ddagger$ & 1.17\,{\scriptsize[1.06, 1.30]} \\
\quad Rescue & 1.60\,{\scriptsize[1.48, 1.73]} & 2.18\,{\scriptsize[1.93, 2.40]} & 2.65\,{\scriptsize[2.45, 2.88]} & 3.57\,{\scriptsize[3.38, 3.78]} \\
\quad Rescue, $W{=}50$ & 2.22\,{\scriptsize[2.08, 2.36]} & 3.22\,{\scriptsize[3.01, 3.44]} & 3.95\,{\scriptsize[3.72, 4.19]} & 4.85\,{\scriptsize[4.50, 5.20]} \\
\quad Rescue, $-5$\,dB & 7.73\,{\scriptsize[7.16, 8.31]} & 9.70\,{\scriptsize[9.04, 10.44]}$^\ddagger$ & 7.66\,{\scriptsize[7.06, 8.29]} & 13.84\,{\scriptsize[12.66, 15.15]} \\


==> figures/table_private.tex <==
Default & 0.37 & 72.9 $\pm$ 6.0 & 69.8 $\pm$ 5.6 & +3.1 [-4.3, +10.7] \\
$W=50$ & 0.62 & 78.4 $\pm$ 7.5 & 73.5 $\pm$ 6.4 & +5.0 [-2.5, +12.8] \\
$\bar\gamma_{\mathrm{ref}}=-5$\,dB & 1.39 & 97.7 $\pm$ 8.4 & 105.0 $\pm$ 9.9 & -7.4 [-17.8, +3.8] \\


==> figures/table_rate_aware.tex <==
Default ($W=100$) & 2 & 66.6 & 22.2 & +2.2 [-3.6, +8.1] & 0.95 & -6.3 [-13.5, +0.9] & 1.84 \\
$W=50$ & 2 & 71.9 & 17.2 & -2.1 [-9.5, +5.5] & 1.08 & -6.5 [-15.3, +2.2] & 2.40 \\
$K=10$ & 2 & 49.9 & 24.2 & +2.0 [-1.8, +5.9] & 0.83 & +3.2 [-0.4, +6.4] & 1.46 \\
Clustered & 2 & 50.8 & 15.7 & +3.6 [-2.3, +9.5] & 0.88 & +1.3 [-4.7, +7.0] & 1.66 \\


==> figures/table_shared_r2.tex <==
Search, $B{=}600$ & 76.2 & 71.8 & +4.4 [-2.5, +10.4] & 13.6 & 74.7 & +1.5 [-4.4, +6.9] & 15.9 & -2.9 [-11.1, +5.3] & 1.16 [1.10, 1.24] & 1.15 [1.09, 1.22] \\
Search, $B{=}300$ & 76.2 & 76.2 & -0.1 [-6.1, +5.9] & 15.8 & 71.3 & +4.9 [-3.0, +11.4] & 15.0 & +4.9 [-3.7, +12.4] & 0.95 [0.89, 1.02] & 1.03 [0.96, 1.10] \\
Search, $B{=}150$ & 76.2 & \multicolumn{8}{c}{target not reached} \\
Rescue, $B{=}300$ & 85.8 & 88.4 & +2.5 [+0.4, +4.7] & 2.1 & 90.0 & +4.2 [+1.9, +6.3] & 10.0 & -1.6 [-4.4, +1.2] & 4.79 [4.43, 5.18] & 4.62 [4.31, 4.95] \\


==> figures/table_validation.tex <==
Search & 76.2 & 70.9 & +5.3 [-2.1, +11.8] & 11.8 & 76.2 & -0.0 [-6.5, +6.1] & 14.0 & -5.3 [-14.8, +4.6] & 1.19 [1.11, 1.27] \\
Search, $K{=}10$ & 57.8 & 54.9 & +2.8 [-2.3, +7.6] & 2.4 & 57.8 & -0.1 [-4.5, +4.1] & 14.5 & -2.9 [-8.8, +3.5] & 5.91 [5.57, 6.29] \\
Search, clustered & 59.0 & 57.8 & +1.2 [-4.1, +6.0] & 6.1 & 55.1 & +3.9 [-2.2, +9.5] & 7.8 & +2.7 [-4.5, +10.0] & 1.28 [1.14, 1.43] \\
\midrule
Rescue & 85.8 & 93.6 & +7.8 [+6.0, +9.4] & 4.1 & 90.0 & +4.2 [+2.0, +6.3] & 7.4 & +3.6 [+1.2, +6.1] & 1.78 [1.63, 1.93] \\
Rescue, $W{=}50$ & 85.8 & 95.1 & +9.3 [+7.8, +10.7] & 3.1 & 87.9 & +2.0 [-0.5, +4.4] & 8.0 & +7.2 [+4.6, +10.0] & 2.60 [2.42, 2.77] \\
Rescue, $-5$\,dB & 85.8 & 89.2 & +3.4 [+1.2, +5.5] & 5.2 & 89.0 & +3.2 [+0.7, +5.4] & 43.9 & +0.2 [-2.6, +3.1] & 8.52 [7.89, 9.19] \\


==> figures/table_values.tex <==
$W=100$ &  5k & 86.4 & +13.4 [+5.4, +23.4] & -0.3 [-8.0, +8.1] & -- \\
$W=100$ &  10k & 74.8 & +12.0 [+4.2, +21.3] & +1.3 [-5.6, +7.7] & +2.6 [-4.5, +19.6] \\
$W=100$ &  20k & 66.4 & +6.9 [+1.9, +12.0] & +3.4 [-2.7, +8.1] & +1.7 [-3.8, +6.0] \\
$W=50$ &  5k & 87.0 & +16.5 [+6.3, +27.5] & -1.6 [-9.9, +8.4] & -- \\
$W=50$ &  10k & 78.4 & +13.4 [-0.5, +26.2] & +2.0 [-4.8, +11.4] & +2.9 [-6.2, +14.8] \\
\midrule
$K=10$ & 5k & 52.1 & +15.3 [+7.9, +21.6] & +1.7 [-3.5, +6.7] & -- \\
$K=10$ & 10k & 51.5 & +11.3 [+4.5, +18.4] & +1.6 [-3.2, +6.3] & -- \\
$K=10$ & 20k & 46.7 & +9.8 [+4.6, +16.6] & +5.0 [+0.9, +7.6] & +0.1 [-3.2, +3.2] \\
Clustered & 5k & 61.9 & +1.9 [-6.8, +10.7] & -5.5 [-11.5, +1.7] & -- \\
Clustered & 10k & 49.1 & +1.9 [-4.6, +8.3] & -0.5 [-6.9, +5.5] & -0.2 [-5.8, +4.9] \\


==> figures/table_where_tom.tex <==
$K=10$ & 5k & 52.1 & +1.7 [-3.5, +6.7] & -- \\
$K=10$ & 10k & 51.5 & +1.6 [-3.2, +6.3] & -- \\
$K=10$ & 20k & 46.7 & +5.0 [+0.9, +7.6] & +0.1 [-3.2, +3.2] \\
\midrule
Clustered & 5k & 61.9 & -5.5 [-11.5, +1.7] & -- \\
Clustered & 10k & 49.1 & -0.5 [-6.9, +5.5] & -0.2 [-5.8, +4.9] \\

